On Blockwise Symmetric Matchgate Signatures and Higher Domain \#CSP

For any $n\geq 3$ and $ q\geq 3$, we prove that the {\sc Equality} function $(=_n)$ on $n$ variables over a domain of size $q$ cannot be realized by matchgates under holographic transformations. This is a consequence of our theorem on the structure of blockwise symmetric matchgate signatures. %due to the rank of the matrix form of the blockwise symmetric standard signatures, %where $(=_n)$ is an equality signature on domain $\{0, 1, \cdots, q-1\}$. This has the implication that the standard holographic algorithms based on matchgates, a methodology known to be universal for \#CSP over the Boolean domain, cannot produce P-time algorithms for planar \#CSP over any higher domain $q\geq 3$.

==> 4-1.tex <==
\subsection{Rank$(\Gamma(1))=1$}
The next lemma shows that
if rank$(\Gamma(1))=1$, then
for all nonzero entries, the indices of all blocks' have the same parity.
%every block of every non-zero entry has the same parity.
\begin{lemma}\label{paritysame }
If rank$(\Gamma(1))=1$ and
there exist
$\alpha_1\alpha_2\cdots\alpha_n$,
$\beta_1\beta_2\cdots\beta_n\in\{0, 1\}^{n\ell}$
such that
 $\Gamma^{\alpha_1\alpha_2\cdots\alpha_n}\neq 0, \Gamma^{\beta_1\beta_2\cdots\beta_n}\neq 0$, then $p(\alpha_i)=p(\beta_j)$ for
$1\leq i, j\leq n$.
%and $\Gamma^{\alpha_k\alpha_k\cdots\alpha_k}\neq 0$
%for $1\leq k\leq n$.
%$, \Gamma^{\alpha_2\alpha_2\cdots\alpha_2}\neq 0,\dots,\Gamma^{\alpha_n\alpha_n\cdots\alpha_n}\neq 0. $
\end{lemma}
\begin{proof}
Note that $p(\alpha_1\alpha_2\cdots\alpha_n)= p(\beta_1\beta_2\cdots\beta_n)$
 by the parity condition of matchgate signatures.
If there exist $i, j$ such that $p(\alpha_i)\neq p(\beta_j)$, then
$p(\alpha_1\cdots\alpha_{i-1}\alpha_{i+1}\cdots\alpha_n)\neq p(\beta_1\cdots\beta_{j-1}\beta_{j+1}\cdots\beta_n)$.
Thus there are two columns in
$
\begin{pmatrix}
\Gamma(1)^{\alpha_i}\\
\Gamma(1)^{\beta_j}
\end{pmatrix}$
of the following form:
\begin{equation*}
\begin{pmatrix}
\Gamma^{\alpha_i\alpha_1\cdots\alpha_{i-1}\alpha_{i+1}\cdots\alpha_n}\\
0
\end{pmatrix},
\begin{pmatrix}
0\\
\Gamma^{\beta_j\beta_1\cdots\beta_{j-1}\beta_{j+1}\cdots\beta_n}
\end{pmatrix}
\end{equation*}
or
\begin{equation*}
\begin{pmatrix}
0\\
\Gamma^{\alpha_i\alpha_1\cdots\alpha_{i-1}\alpha_{i+1}\cdots\alpha_n}
\end{pmatrix},
\begin{pmatrix}
\Gamma^{\beta_j\alpha_1\cdots\beta_{j-1}\beta_{j+1}\cdots\beta_n}\\
0
\end{pmatrix}
\end{equation*}
that are linearly independent.
This implies that $\Gamma(1)$ has a submatrix of rank 2.
It contradicts the fact that rank$(\Gamma(1))=1$.
\end{proof}
Now we prove Theorem~\ref{fu'stheorem1} for the case that rank$(\Gamma(1))=1$.

\begin{theorem}\label{dege}
Let $\Gamma=(\Gamma^{\alpha_1\alpha_2\cdots\alpha_n})$ be a blockwise symmetric signature of arity $n\ell$, where $n\geq 3$.
If $\Gamma$ is realized by a matchgate and rank$(\Gamma(1))=1$,
then  there exists a condensed signature $(g_{\alpha})_{\alpha\in\{0, 1\}^{\ell}}$ that is realized by a matchgate with arity $\ell+1$,
and $\beta\in\{0, 1\}^{\ell}$ such that
\begin{equation}\label{dege-2}
\Gamma^{\alpha_{1}\alpha_{2}\cdots\alpha_{n}}
=g_{\alpha_{1}}g_{\alpha_{2}}\cdots g_{\alpha_{n}}\Gamma^{\beta\beta\cdots\beta}.
\end{equation}

Moreover, there is a bitwise symmetric matchgate signature $\Gamma_{S}$ that is realized by a matchgate with arity $n$ such that
\begin{equation}\label{dege-3}
\Gamma^{\alpha_{1}\alpha_{2}\cdots\alpha_{n}}
=g_{\alpha_{1}}g_{\alpha_{2}}\cdots g_{\alpha_{n}}\Gamma_{S}^{p(\alpha_{1})p(\alpha_{2})\cdots p(\alpha_{n})}.
\end{equation}
\end{theorem}

\begin{proof}
Since rank$(\Gamma(1))=1$, there exists
$\beta_1\beta_2\cdots\beta_n\in\{0, 1\}^{n\ell}$
such that
$\Gamma^{\beta_1\beta_2\cdots\beta_n}\neq 0$.
After a global factor, we can assume that $\Gamma^{\beta_1\beta_2\cdots\beta_n}=1$.
So %the $\beta_1$-th row of $\Gamma(1)$
we have $\Gamma(1)^{\beta_1}\neq 0$. Thus for any $\alpha_i\in\{0, 1\}^{\ell}$, there exists
$g_{\alpha_i}$ such that $\Gamma(1)^{\alpha_i}=g_{\alpha_i}\Gamma(1)^{\beta_1}$
by rank$(\Gamma(1))=1$.
Note that $g_{\alpha}=\Gamma^{\alpha\beta_2\cdots\beta_n}$ for any $\alpha\in\{0, 1\}^{\ell}$.
%Let $\beta=\beta_1$.

Firstly, we prove that $g=(g_{\alpha})$ is a condensed signature.
Assume that $\Gamma=(\Gamma^{\alpha_1\alpha_2\cdots\alpha_n})$ is realized by the matchgate
$G$ with arity $n\ell$.
Note that $G$ has $n\ell$ external nodes
and we group the external nodes into $n$ blocks of
%%% JYC edits
%%%%%%I am not sure we can use "each" in this way--Zhiguo
consecutive $\ell$ nodes each.
%We view the external nodes of $\Gamma$ as $n$ blocks.
We do nothing to the first block of $G$.
%If $p(\beta_1)=0$, we do noting to the first external node of the second block.
%If $p(\beta_1)=1$, we connect an edge with weight 1 to the first external node of the second block of
%$\Gamma$ and take the new vertex as external node.
%For other external nodes, we make the following changes:
For the $i$-th block, where $2\leq i\leq n$,
if the $j$-th bit of $\beta_i$
is 0, do nothing to $G$; if the $j$-th bit of $\beta_i$
is 1, connect an edge with weight 1 to the $j$-th
external node of the $i$-th block of
$G$ and take the new vertex as external node.
Then we get a new matchgate $G'$.
For $G'$, view the external nodes of the first block and the first
external node of the second block as external nodes and all other nodes as
internal nodes, then we get a new matchgate $G''$ with arity $\ell+1$.
Recall that $g_\alpha=\Gamma^{\alpha\beta_2\cdots\beta_n}$. Thus $g$ is the
condensed signature of $G''$.

Let
$\beta=\beta_1$.
For any $\Gamma^{\alpha_1\alpha_2\cdots\alpha_n}$,
we prove (\ref{dege-2}) by  induction on $t$,
defined to be the number of $\alpha_i$ that are not equal to $\beta_1$ in $\{\alpha_1, \alpha_2, \cdots, \alpha_n\}$.
Note that $g_{\beta_1}=1$.
If all of $\alpha_i$
are equal to $\beta_1$ in $\{\alpha_1, \alpha_2, \cdots, \alpha_n\}$, i.e., $t=0$, then (\ref{dege-2}) is already valid.
Inductively we assume that (\ref{dege-2}) has been proved for $t-1$
and there are $t\geq 1$ blocks
that are not equal to $\beta_1$ in $\{\alpha_1, \alpha_2, \cdots, \alpha_n\}$.
Thus there exists at least one
$\alpha_i\neq\beta_1$ in $\{\alpha_1, \alpha_2, \cdots, \alpha_n\}$.
If $p(\alpha_i)\neq p(\beta_1)$, then $g_{\alpha_i}=0$ and $\Gamma^{\alpha_1\cdots\alpha_i\cdots\alpha_n}=0$ by Lemma~\ref{paritysame }.
Thus we are done.
For $p(\alpha_i)=p(\beta_1)$, the $\alpha_i$-th row $\Gamma(1)^{\alpha_i}=g_{\alpha_i}\Gamma(1)^{\beta_1}$ in
\begin{equation*}
\Gamma(1)=\begin{pmatrix}
\cdots&\cdots&\cdots\\
\cdots&\Gamma^{\beta_1\alpha_1\cdots\alpha_{i-1}\alpha_{i+1}\cdots\alpha_n}&\cdots\\
\cdots&\cdots&\cdots\\
\cdots&\Gamma^{\alpha_i\alpha_1\cdots\alpha_{i-1}\alpha_{i+1}\cdots\alpha_n}&\cdots\\
\cdots&\cdots&\cdots
\end{pmatrix}.
\end{equation*}
Thus
\[\Gamma^{\alpha_1\alpha_2\cdots\alpha_n}=\Gamma^{\alpha_i\alpha_1\cdots\alpha_{i-1}\alpha_{i+1}\cdots\alpha_n}=
g_{\alpha_i}\Gamma^{\beta_1\alpha_1\cdots\alpha_{i-1}\alpha_{i+1}\cdots\alpha_n}.\]
 Note that
the number of blocks that are not equal to $\beta_1$ in $\{\beta_1, \alpha_1, \cdots, \alpha_{i-1}, \alpha_{i+1}, \cdots, \alpha_n\}$ is
$t-1$. By induction, we
have
\[
\Gamma^{\beta_1\alpha_1\cdots\alpha_{i-1}\alpha_{i+1}\cdots\alpha_n}=g_{\alpha_1}\cdots g_{\alpha_{i-1}}g_{\alpha_{i+1}}\cdots g_{\alpha_n}
\Gamma^{\beta_1\beta_1\cdots\beta_1}.
\]
So we have
\begin{equation}\label{tensor-equation}
\Gamma^{\alpha_1\alpha_2\cdots\alpha_n}=
g_{\alpha_1}g_{\alpha_2}\cdots g_{\alpha_n}
\Gamma^{\beta_1\beta_1\cdots\beta_1}.\end{equation}
This finishes the proof of (\ref{dege-2}).

Let $\lambda=\sqrt[n]{\Gamma^{\beta_1\beta_1\cdots\beta_1}}$.
For $p(\beta_1)=0$, let $\Gamma_S=(\lambda, 0)^{\otimes n}$,
then $\Gamma_S$ is realized by $n$ copies of the matchgate $\Gamma_1$.

\setlength{\unitlength}{2.3mm}
\begin{picture}(30,7)(0,0)
\put(31,4){\line(1, 0){10}}
\put(30.8,3.5){$\bullet$}
\put(40.8,3.5){$\bullet$}
\put(35, 5){\rm \scriptsize $\lambda$}
\put(8, 2){\rm \scriptsize $\Gamma_1$: The left node is the external node and the other node is the internal node.
The edge has weight $\lambda$.}
\end{picture}
\newline
For $p(\beta_1)=1$, let $\Gamma_S=(0, \lambda)^{\otimes n}$,
then $\Gamma_S$ is realized by $n$ copies of the matchgate $\Gamma_2$.

\setlength{\unitlength}{2.3mm}
\begin{picture}(30,8)(0,-1)
\put(26,4){\line(1, 0){20}}
\put(25.8,3.5){$\bullet$}
\put(35.8,3.5){$\bullet$}
\put(45.8,3.5){$\bullet$}
\put(40, 5){\rm \scriptsize $\lambda$}
\put(30, 5){\rm \scriptsize 1}
\put(13, 2){\rm \scriptsize $\Gamma_2$: The leftmost node is the external node and the other nodes are internal nodes.}
\put(15, 0){\rm \scriptsize The left edge has weight 1 and the right edge has weight $\lambda$.}
\end{picture}
\newline
Note that all the entries of $\Gamma_S$ are zero except
$\Gamma_S^{p(\beta_1)p(\beta_1)\cdots p(\beta_1)}=\Gamma^{\beta_1\beta_1\cdots\beta_1}$.
For any entry $\Gamma^{\alpha_1\alpha_2\cdots\alpha_n}$
of $\Gamma$, if there is $\alpha_i$ such that $p(\alpha_i)\neq p(\beta_1)$
in $\{\alpha_1, \alpha_2, \cdots, \alpha_n\}$,
then $\Gamma^{\alpha_1\alpha_2\cdots\alpha_n}=0$ by Lemma~\ref{paritysame }.
Thus we have
\[\Gamma^{\alpha_1\alpha_2\cdots\alpha_n}=
g_{\alpha_1}g_{\alpha_2}\cdots g_{\alpha_n}
\Gamma_S^{p(\alpha_1)p(\alpha_2)\cdots p(\alpha_n)}=0.\]
If $p(\alpha_i)=p(\beta_1)$ for $1\leq i\leq n$, we directly have
\[\Gamma^{\alpha_1\alpha_2\cdots\alpha_n}=
g_{\alpha_1}g_{\alpha_2}\cdots g_{\alpha_n}
\Gamma_S^{p(\alpha_1)p(\alpha_2)\cdots p(\alpha_n)}\]
by (\ref{tensor-equation}).
\end{proof}



==> 4-2.tex <==
\section{The structure of blockwise symmetric matchagate signatures}
For an $n$-bit string $\alpha\in\{0, 1\}^{n}$, we define $p(\alpha)=0$ if wt$(\alpha)$ is even and $p(\alpha)=1$ if wt$(\alpha)$ is odd.

\begin{definition}{\rm
For an even (resp. odd) matchgate $\Gamma$ with arity $n$, the {\it condensed signature} $(g_{\alpha})$  of $\Gamma$
is a vector of dimension $2^{n-1}$, and $g_{\alpha}=\Gamma^{\alpha b}$ (resp. $g_{\alpha}=\Gamma^{\alpha\bar{b}}$),
where $\alpha\in\{0, 1\}^{n-1}$ and $b=p(\alpha)$.}
\end{definition}

For the structure of the blockwise symmetric matchgate signatures,
the following theorem  was given in \cite{cailu10}.
\begin{theorem}\label{cai'stheorem1}
Let $\Gamma=(\Gamma^{\alpha_{1}\alpha_2\cdots\alpha_n})$ be a blockwise symmetric signature
%with block size $2$
with arity $n\ell$, where $n\geq 4$.
If $\Gamma$ is realized by an even matchgate (resp. odd matchgate) and $\Gamma^{\mathbf{0}\mathbf{0}\cdots \mathbf{0}}\neq 0$
(resp. $\Gamma^{e_1 \mathbf{0}\cdots \mathbf{0}}\neq 0$),
 %Assume that $n\geq 4$ and $\Gamma^{00\cdots 0}\neq 0$($\Gamma^{e_{1}0\cdots 0}\neq 0$).
 %then $\Gamma$ is realizable by a matchgate iff
then  there exists a condensed signature $(g_{\alpha})_{\alpha\in\{0, 1\}^{\ell}}$ that is realized by a matchgate with arity $\ell+1$, and a bitwise symmetric matchgate signature $\Gamma_{S}$ that is realized by a matchgate with arity $n$ such that
\begin{equation}
\Gamma^{\alpha_{1}\alpha_{2}\cdots\alpha_{n}}
=g_{\alpha_{1}}g_{\alpha_{2}}\cdots g_{\alpha_{n}}\Gamma_{S}^{p(\alpha_{1})p(\alpha_{2})\cdots p(\alpha_{n})}.
\end{equation}
\end{theorem}

Furthermore, Theorem \ref{cai'stheorem1} is proved for the blockwise symmetric matchgate signatures of block size $\ell=2$ without the condition
 $\Gamma^{\mathbf{0}\mathbf{0}\cdots \mathbf{0}}\neq 0$ in \cite{cailu10},
but the authors pointed out that the proof is ``relentless", \ldots, ``A better and more conceptual proof
would be very desirable and lead to a better understanding of realizable signatures."
and ``Whether one can remove the technical condition $\Gamma^{\mathbf{0}\mathbf{0}\cdots \mathbf{0}}\neq 0$ for signatures with block size greater than 2 is an interesting open problem."
In the present paper, the following theorem is proved:

\begin{theorem}\label{fu'stheorem1}
Let $\Gamma=(\Gamma^{\alpha_{1}\alpha_2\cdots\alpha_n}$) be a blockwise symmetric sigature
%with block size $2$
with arity $n\ell$, where $n\geq 3$.
If $\Gamma$ is realized by a matchgate,
then  there exists a condensed signature $(g_{\alpha})_{\alpha\in\{0, 1\}^{\ell}}$ that is realized by a matchgate with arity $\ell+1$, and a bitwise symmetric matchgate signature $\Gamma_{s}$ that is realized by a matchgate with arity $n$ such that
\begin{equation}
\Gamma^{\alpha_{1}\alpha_{2}\cdots\alpha_{n}}
=g_{\alpha_{1}}g_{\alpha_{2}}\cdots g_{\alpha_{n}}\Gamma_{S}^{p(\alpha_{1})p(\alpha_{2})\cdots p(\alpha_{n})}.
\end{equation}
\end{theorem}
Theorem \ref{fu'stheorem1} can work for the signatures  of general block size without the non-zero condition.
Moreover, it only requires that the number of blocks is  $n\geq 3$ instead of $n\geq 4$.
 The example in the end of Section~\ref{main-section} shows that Theorem \ref{fu'stheorem1} can not work for
$n=2$. Thus we give a complete characterization of the structure of the blockwise symmetric matchgate signatures.

The proof in \cite{cailu10} is by induction on the Hamming weight of $\alpha_1\alpha_2\cdots\alpha_n$.
To reduce to the entries of  lower Hamming weight, the proof uses MGI and $\Gamma^{\mathbf{0}\mathbf{0}\cdots\mathbf{0}}\neq 0$
or $\Gamma^{e_1\mathbf{0}\cdots\mathbf{0}}$.
This is why they can not remove the non-zero condition.
In the present paper, we use the matrix form of a matchgate signature.
We prove that the matrix form of a blockwise symmetric matchgate signature has rank at most 2.
This is the reason that the blockwise symmetric matchgate signature has the special form in Theorem~\ref{fu'stheorem1}.
The proof heavily depends on MGI as \cite{cailu10}, but it is not an induction on Hamming weight.
So it does not need the non-zero condition.

By Lemma~\ref{mainlemma}, rank$(M(\Gamma))=0, 1$ or 2.
If rank$(\Gamma(1))=0$, then the signature is identically zero
and Theorem~\ref{fu'stheorem1} follows directly. In the following, we prove Theorem \ref{fu'stheorem1} for rank($\Gamma(1)$)=2 and omit the proof for
rank($\Gamma(1)$)=1 due to the space limit.


%\subsection{Rank($\Gamma(1)$)=2}
%Now we prove Theorem~\ref{fu'stheorem1} for the case that rank$(\Gamma(1))=2$.
%By Theorem~\ref{mainlemma}, this finishes the proof of Theorem~\ref{fu'stheorem1}.

\begin{theorem}\label{maintheorem}
Let $\Gamma=(\Gamma^{\alpha_{1}\alpha_2\cdots\alpha_n}$) be a blockwise symmetric signature
%with block size $2$
with arity $n\ell$, where $n\geq 3$.
If $\Gamma$ is realized by a matchgate and rank$(\Gamma(1))=2$,
then  there exists a condensed signature $(g_{\alpha})_{\alpha\in\{0, 1\}^{\ell}}$ that is realized by a matchgate with arity $\ell+1$, and a bitwise symmetric matchgate signature $\Gamma_{S}$ that is realized by a matchgate with arity $n$ such that
\begin{equation}\label{xxxx}
\Gamma^{\alpha_{1}\alpha_{2}\cdots\alpha_{n}}
=g_{\alpha_{1}}g_{\alpha_{2}}\cdots g_{\alpha_{n}}\Gamma_{S}^{p(\alpha_{1})p(\alpha_{2})\cdots p(\alpha_{n})}.
\end{equation}
\end{theorem}
\begin{proof}
By Lemma~\ref{le-col-2-1}, $\Gamma(1)$ has a full rank submatrix of the following form
%\[
%\begin{pmatrix}
%\Gamma^{\theta\gamma_{2}\cdots\gamma_{n}}&0\\
%0&\Gamma^{\eta(\gamma_{2}\cdots\gamma_{n}+e_p)}
%\end{pmatrix}
%{\rm or}
%\begin{pmatrix}
%0&\Gamma^{\theta\gamma_{2}\cdots\gamma_{n}}\\
%\Gamma^{(\eta(\gamma_{2}\cdots\gamma_{n}+e_p)}&0
%\end{pmatrix},
%\]
%where $\theta+\eta=e_s\in\{0, 1\}^{\ell}$ and $e_p\in\{0, 1\}^{(n-1)\ell}$.
%Note that $\Gamma$ is blockwise symmetric.
%Thus for any entry $\Gamma^{\alpha_1\alpha_2\cdots\alpha_n}$, we can adjust the order of the blocks freely.
%So we can assume that $\Gamma(1)$ has a full rank submatrix of the following form
\[\begin{pmatrix}
\Gamma^{\theta\gamma_{2}\cdots\gamma_{n}}&0\\
0&\Gamma^{\eta(\gamma_{2}+e_{t})\cdots\gamma_{n}}
\end{pmatrix}~~~~~~~
{\rm or }~~~~~~\begin{pmatrix}
0&\Gamma^{\theta\gamma_{2}\cdots\gamma_{n}}\\
\Gamma^{\eta(\gamma_{2}+e_{t})\cdots\gamma_{n}}&0
\end{pmatrix},\]
where $\theta, \eta, \gamma_j\in\{0, 1\}^{\ell}$ for $2\leq j\leq n$ and $\theta+\eta=e_{s}$,
where $e_s, e_t\in\{0, 1\}^{\ell}$.
Note that $p(\theta)\neq p(\eta)$.
Without loss of generality, we assume that $p(\theta)=0$ and $p(\eta)=1$ in the following.
%In the following, we assume that the $s$-th bit of $\gamma_2$ is 1.
%Otherwise, we only need to swich the roles of $\alpha$ and $\beta$, $\gamma_2$ and $\gamma_2+e_s$ respectively.


%Note that $G^{\alpha\alpha_{2}\cdots\alpha_{n}}\neq 0, G^{\beta(\alpha_{2}+e_{s})\cdots\alpha_{n}}\neq 0$.
Note that the rows $\Gamma(1)^{\theta}$ and $\Gamma(1)^{\eta}$ are linearly independent.
Then by rank$(\Gamma(1))=2$, all of the rows of $\Gamma(1)$ are linear combinations of  $\Gamma(1)^{\theta}$ and $\Gamma(1)^{\eta}$.
%$\Gamma(1)^{\alpha_{i}}=\lambda \Gamma(1)^{\alpha}$+$\mu \Gamma(1)^{\beta}$ for any $\alpha_{i}\in\{0, 1\}^{\ell}$.
Moreover,  for any $\alpha_i, \alpha_j\in\{0, 1\}^{\ell}$, by the parity condition of $\Gamma$, if $p(\alpha_i)\neq p(\alpha_j)$,
the nonzero entries of $\Gamma(1)^{\alpha_{i}}$ and $\Gamma(1)^{\alpha_{j}}$
are in disjoint column positions.
So $\Gamma(1)^{\alpha_{i}}$ and $\Gamma(1)^{\alpha_{j}}$ are orthogonal. Thus for any $\alpha\in\{0, 1\}^{\ell}$
there exists $g_{\alpha}$  such that
$\Gamma(1)^{\alpha}=g_{\alpha} \Gamma(1)^{\theta}$ if $p(\alpha)= p(\theta)$,
and $\Gamma(1)^{\alpha}=g_{\alpha} \Gamma(1)^{\eta}$ if $p(\alpha)= p(\eta)$.

Up to a global nonzero scalar, we can assume that $\Gamma^{\theta\gamma_2\cdots\gamma_n}=1$ and $\Gamma^{\eta(\gamma_2+e_t)\cdots\gamma_n}=r$, then
for any $\alpha\in\{0, 1\}^{\ell}$,
$g_{\alpha}=\Gamma^{\alpha\gamma_2\cdots\gamma_n}$ if $p(\alpha)=p(\theta)$, and
$g_{\alpha}=r^{-1}\Gamma^{\alpha(\gamma_2+e_t)\cdots\gamma_n}$ if $p(\alpha)=p(\eta)$.
Now we prove that $g=(g_{\alpha})$ is a condensed signature.
Assume that $\Gamma=(\Gamma^{\alpha_1\alpha_2\cdots\alpha_n})$ is realized by the matchgate
$G$ with arity $n\ell$.
%Let $\Gamma$ be the matchgate realizing the matchgate signature $\Gamma=(\Gamma^{\alpha_1\alpha_2\cdots\alpha_n})$.
Note that $G$ has $n\ell$ external nodes
and we group the external nodes into $n$ blocks of
%%% JYC edits
%%%%%%I am not sure we can use "each" in this way--Zhiguo
consecutive $\ell$ nodes each.
Firstly, we connect a path $L$ of length 2 to
the $(\ell+t)$-th external node, i.e., the $t$-th node of the second block, of $G$.
We denote the $(\ell+t)$-th external node of $G$, i.e., one endpoint of $L$, as $v_1$,
another endpoint of $L$ as $v_3$ and the middle node of $L$ as $v_2$.
If the $(\ell+t)$-th bit of $\theta\gamma_2\cdots\gamma_n$ is 0, we give the edge between
$v_1$ and $v_2$ weight $r^{-1}$ and the edge between
$v_2$ and $v_3$ weight 1.
If the $(\ell+t)$-th bit of $\theta\gamma_2\cdots\gamma_n$ is 1, we give the edge between
$v_1$ and $v_2$ weight 1 and the edge between
$v_2$ and $v_3$ weight $r^{-1}$, and view $v_3$ as an external node and $v_1, v_2$ as internal nodes.
We do nothing to the external nodes in the  first block and still view them as external nodes.
We view other external nodes, i.e., the external nodes that are not in the first block and not the $(\ell+t)$-th external node,
as internal node and do the following operations to them:
for $\ell+1\leq i\leq n\ell$ and $i\neq \ell+t$,
 if the $i$-th bit of $\theta\gamma_2\cdots\gamma_n$
is 0, do nothing to $G$; if the $i$-th bit of $\theta\gamma_2\cdots\gamma_n$
is 1, connect an edge with weight 1 to the $i$-th
external node of $G$ and view the new nodes as internal nodes.
Then we get a new matchgate $G'$ with arity $\ell+1$ and $g$ is the
condensed signature of $G'$.

Now we construct the matchgate signature $\Gamma_S$ of arity $n$.
For every block of $G$, for  $1\leq i\leq \ell$,
 if the $i$-th bit of $\theta$ is 1
then  we add an edge
 of weight 1 to the $i$-th external node,
and the new node replaces it as an external node.
 If the $i$-th bit of $\theta$ is 0
then we do nothing to it.
We get a new matchgate $H$.
Note that all the bits of $\theta, \eta$ are the same except the $s$-th bit.
Next, we define  $H'$ from  $H$:
 In each block of  $\ell$ external nodes of $H$,
we pick only the $s$-th external node as an external node
of $H'$; all others are considered internal nodes of
$H'$.
We denote the matchgate signature of  $H'$
by $\Gamma_{S}$.
Then
 $\Gamma_S=(\Gamma_{S}^{j_1 j_2 \cdots j_n})$
is a signature of arity $n$
and
$\Gamma_S^{j_1j_2\cdots j_n}=\Gamma^{\alpha_1 \alpha_2\cdots \alpha_n}$, where $\alpha_i\in\{\theta, \eta\}$ and
$j_i=p(\alpha_i)$.

Now for any $\alpha_1\alpha_2\cdots\alpha_n\in\{0, 1\}^{n\ell}$, we prove (\ref{xxxx}) by  induction on $t$,
 the number of $\alpha_i$ from $\{\alpha_1, \alpha_2, \cdots, \alpha_n\}$ that do not belong to $\{\theta, \eta\}$ in $\{\alpha_1, \alpha_2, \ldots, \alpha_n\}$.
Note that $g_{\theta}=g_{\eta}=1$.
If all $\alpha_i$ are among $\{\theta, \eta\}$, i.e., $t=0$, we are done by the definition of $\Gamma_{S}^{j_1 j_2 \cdots j_n}$
and (\ref{xxxx}) is proved.
Inductively we assume that (\ref{xxxx}) has been proved for $t-1$
and there are $t\geq 1$ blocks in $\{\alpha_1, \alpha_2, \ldots, \alpha_n\}$
that are not among $\{\theta, \eta\}$.
Then there is at least one $\alpha_i$  that is not among $\{\theta, \eta\}$.
If  $\alpha_i$ has the same parity as $\theta$, then
the $\alpha_i$-th row $\Gamma(1)^{\alpha_i}=g_{\alpha_i}\Gamma(1)^{\theta}$
in
\begin{equation*}
\Gamma(1)=\begin{pmatrix}
\cdots&\cdots&\cdots\\
\cdots&\Gamma^{\theta\alpha_1\cdots\alpha_{i-1}\alpha_{i+1}\cdots\alpha_n}&\cdots\\
\cdots&\cdots&\cdots\\
\cdots&\Gamma^{\alpha_i\alpha_1\cdots\alpha_{i-1}\alpha_{i+1}\cdots\alpha_n}&\cdots\\
\cdots&\cdots&\cdots
\end{pmatrix}.
\end{equation*}
Thus
 \[\Gamma^{\alpha_1\alpha_2\cdots\alpha_n}=\Gamma^{\alpha_i\alpha_1\cdots\alpha_{i-1}\alpha_{i+1}\cdots\alpha_n}=
g_{\alpha_i}\Gamma^{\theta\alpha_1\cdots\alpha_{i-1}\alpha_{i+1}\cdots\alpha_n}.\]
Note that
the number of blocks from $\{\theta, \alpha_1, \cdots, \alpha_{i-1}, \alpha_{i+1}, \cdots, \alpha_n\}$ that do not belong to $\{\theta, \eta\}$ is
$t-1$. Thus we have
\[
\Gamma^{\theta\alpha_1\cdots\alpha_{i-1}\alpha_{i+1}\cdots\alpha_n}=g_{\alpha_2}\cdots g_{\alpha_{i-1}}g_{\alpha_{i+1}}\cdots g_{\alpha_n}
\Gamma_S^{p(\theta) p(\alpha_2)\cdots p(\alpha_n)}
\]
by induction.
Then
\[\Gamma^{\alpha_1\alpha_2\cdots\alpha_n}=
g_{\alpha_1}g_{\alpha_2}\cdots g_{\alpha_n}
\Gamma_S^{p(\alpha_1)p(\alpha_2)\cdots p(\alpha_n)}\]
 and we complete the proof.

If $p(\alpha_i)=p(\eta)$, the proof is similar and we omit it here.
\end{proof}




%By Theorem~\ref{mainlemma}, Theorem~\ref{dege} and Theorem~\ref{maintheorem}, we finish the proof of Theorem~\ref{fu'stheorem1}.



==> ACK.tex <==
\section{Acknowlegements}
I am very grateful to Prof. Jin-Yi, Cai for his guidance and discussions.

